Deep KKL: Data-driven Output Prediction for Non-Linear Systems

We address the problem of output prediction, ie. designing a model for autonomous nonlinear systems capable of forecasting their future observations. We first define a general framework bringing together the necessary properties for the development of such an output predictor. In particular, we look at this problem from two different viewpoints, control theory and data-driven techniques (machine learning), and try to formulate it in a consistent way, reducing the gap between the two fields. Building on this formulation and problem definition, we propose a predictor structure based on the Kazantzis-Kravaris/Luenberger (KKL) observer and we show that KKL fits well into our general framework. Finally, we propose a constructive solution for this predictor that solely relies on a small set of trajectories measured from the system. Our experiments show that our solution allows to obtain an efficient predictor over a subset of the observation space.

==> sections/math_proof.tex <==
\section{APPENDIX}
\subsection{Proof of Proposition \ref{prop1}}
\label{proof_prop1}
Because of the triangular structure of \ref{eq:kkl}, $Z(x,z,t)$ is defined $\forall t,x,z\in \RR^+\times\mO\times\CC^m$ as long as $h(X(x,t))$ is defined, which is the case for $t>0$, hence $(X(x,t), Z(x,z,t))$ is defined for $t>0$.

From \ref{eq:assumption1} and \ref{eq:kkl}, we obtain for each $x,z\in \mO\times \CC^m$, and $t>0$
$$T(X(x,t)) - Z(x,z,t) = e^{At}(T(x) - z)$$
As $A$ is Hurwitz, we have
$$\lim_{t\rightarrow\infty} |Z(x,z,t) - T(X(x,t))| = 0$$

From this, \ref{eq:result1} follows readily if there exists a continuous function $\psi$ and a class $\kappa^\infty$ function $\rho^*$ satisfying 
$$|\psi(z) - x| \leq \rho^*(|z-T(x)|)\quad \forall (x,z)\in \mO\times\CC^m$$

To find such function, we first remark that, for all $z\in \CC^m$, the function $x\mapsto |z-T(x)|$ is continuous on the compact $\mO$ (since $T$ is continuous). Then, this function is bounded and the minimum is reached by at least one point noted $T^*(z)\in \mO$.

This defines a function $T^*:\CC^m\mapsto \mO$ satisfying
\begin{equation}
    \label{eq:minTp}
    T(T^*(z)) = z \quad \forall z \in T(\mO)
\end{equation}
\begin{equation}
    \label{eq:proof1_ineq}
    |T(T^*(z)) - z| \leq |T(x)-z| \quad \forall (x,z)\in \mO\times\CC^m
\end{equation}

\sj{Normally, that is the moment where we show that injectivity of T brings continuity of $T^*$ (which is easy), but $T$ is not injective anymore ! and I can't find a proof using \ref{eq:assumption2} and \ref{eq:minTp} that bring continuity without assuming that $h$ is injective. So here we loose continuity of $\psi$ !}

Hence, using \ref{eq:assumption2}, for all $x\in \mO$ and $z\in \CC^m$ :
$$|h(T^*(z)) - h(x)| \leq \rho(|T(T^*(z)) - z|+|z-T(x)|)$$
Then, by injecting \ref{eq:proof1_ineq} 
$$|h(T^*(z))-h(x)| \leq 2\rho(|T(x)-z|)$$
Since this result is true for each $(z,x)$, it is also true for $(X(x,t), Z(x,z,t))$ for all $t>0$. Then, we obtain \ref{eq:result1} by introducing $\psi = h\circ T^*$:
$$\lim_{t\mapsto \infty}|\psi(Z(x,z,t)) - h(X(x,t))| =0$$
\begin{flushright}
\QED
\end{flushright}

\sj{The proof should be longuer, since we should need to construct a smooth solution on $\CC^m\setminus T(\mO)$, but since we can't prove that $T^*$ is continuous, it is not needed for now.}

\subsection{Proof of Proposition \ref{prop2}}
\label{proof_prop2}
Since $\mO$ is invariant, $X(x,s)\in \mO$ for all $x\in \mO$ and $t<0$. Moreover, $\mO$ is bounded (compact in $\RR^n$) then $X(x,s)$ is bounded. In addition, $h$ is continuous on $\mO$ closed and bounded, hence it is bounded too. Then, there exists $K \in \RR^+$ such that :
$$|e^{-As}bh(X(x,s))| \leq K|e^{-As}|$$
which is integrable on $\RR^-$.

\sj{The proof in the paper is much more complex than this, but I think that $\mO$ compact simplify the story. Nevertheless, I still struggle to prove that $T$ is continuous. The paper use the Lesbegue dominated convergence, which do not statuate on continuity as far as I understand. \\
I want to use the theorem "Continuity under the integral", but to do that, I need to prove that $f(s,x) = e^{-As}bh(X(x,s))$ is continuous with regards to $x$ and $t$. It seems trivial in the paper, but it is not for me !}

Then $T$ defined as \ref{eq:T} is well defined and continuous on $\mO$. Now for each $x\in\mO$ and $t\in \RR^-$ 
$$T(X(x,t))-T(x) = \int_{-\infty}^0 e^{-As}bh(X(X(x,t),s))ds - T(x)$$

So
\begin{multline*}
    T(X(x,t)) - T(x) = (e^{At}-1)T(x) \\+ e^{At}\int_0^t e^{-Au}bh(X(x,u))du
\end{multline*}
Then, it follows that
$$L_f T = \lim_{t\rightarrow 0} \frac{T(X(x,t))-T(x)}{t} = AT(x) +bh(x)$$

\begin{flushright}
\QED
\end{flushright}

\subsection{Proof of proposition \ref{prop3}}
Consider $A = \text{diag}(\lambda_1, ..., \lambda_{n+1})$ and $b=(\beta, \, ..., \beta)^T$ with $\lambda_i \in \CC_l = \{\lambda\in \CC, \, Re(\lambda)<-l\}$. It turns out that 
$$T(z) = \left[\begin{array}{c}
     T_1(z) \\
     \vdots \\
     T_{n+1}(z)
\end{array}\right] \quad T_i(z) = \int_{-\infty}^0 e^{-\lambda_i s}\beta h(X(x,s))ds$$
We will prove that there exists an $l>0$ such that by arbitrarily choosing $\lambda \in \CC_L\setminus\mS$ where $\mS$ is a set of zero Lebesgue measure, the map $T$ is such that
$$T(x_1)=T(x_2) \Rightarrow h(x_1)=h(x_2) \quad \forall (x_1, x_2)\in \mO^2$$
More precisely, we will prove that having defined $\mY = \{(x_1,x_2)\in \mO^2, \, h(x_1)\neq h(x_2)\}$, the set $\mS = \{(\lambda_1, ..., \lambda_{n+1})\in \CC_l^{n+1}, \, \exists (x_1, x_2)\in \mY \text{ such that } T_i(x_1)=T_i(x_2)\,\forall i\}$ has a zero Lebesgue measure for a proper choice of $l$.

To this end, Lemma \ref{coron} plays a crucial role.

\begin{lemma}
\label{coron} Let $\Omega$ and $\mY$ be open subsets of $\CC$ and $\RR^{2n}$ respectively. Let 
$$\delta_T : \left\{\begin{array}{l}
     \mY\times \Omega \mapsto \CC \\
    \omega, \lambda \mapsto \delta_T(\omega, \lambda)
\end{array}\right.$$
be an holomorphic function in $\lambda$ for all $\omega\in \mY$ and $C^1$ in $\omega$ for all $\lambda\in\Omega$.

If, for each pair $\omega\in \mY$, the function $\lambda \mapsto \delta_T(\omega, \lambda)$ is not identically zero on $\Omega$, then the set 
$$\mS = \cup_{\omega\in \mY} \{(\lambda_1, ..., \lambda_{n+1})\in \CC_l^{n+1}, \, \delta_T(\omega, \lambda_i)=0\, \forall i\}$$
has a zero Lebesgue measure.
\end{lemma}

Before that, we need to prove $T$ is $C^1$. This is achieve with Lemma \ref{c1}

\begin{lemma}
\label{c1} There exists an $l>0$ such that for all $\lambda_i\in \CC_l$, $T$ is $C^1$.
\end{lemma}
\begin{proof}
This is an application of the theorem of derivation under the integral. We need to verify that, if $f(x,s) = e^{-\lambda s}\beta h(X(x,s))$ 
\begin{enumerate}
    \item $\forall x \in \mO$, $t\mapsto f(x,t)$ is continuous piecewise on $\RR^-$ and integrable
    \item $\forall t \in \RR^-$, $x\mapsto f(x,t)$ is $C^1$ on $\mO$
    \item $\forall x\in \mO$, $t\mapsto \frac{\partial f}{\partial x}(t,s)$ is continuous piecewise 
    \item There exists an integrable function $\psi$ such that $\left|\frac{\partial f}{\partial x}\right| \leq \psi(t)$
\end{enumerate}

\sj{Assuming that condition 1 and 2 are already satisfied because $T$ is continuous (which is a hard point for me, cf previous comment), I still have some problem with condition 3. The paper only describe how to verify condition 4.}

Lets prove that $e^{-\lambda s}\beta \frac{\partial h}{\partial x}(X(x,s))$ is integrable. Consider :
$$\frac{\partial }{\partial x}(h(X(x,s)) = \frac{\partial h}{\partial x}(X(x,s)) \frac{\partial X}{\partial x}(x,s)$$
Since $\mO$ is compact, $\exists M > 0$ such that $X(x,s)\leq M$ for all $(x,s)\in \mO\times\RR^-$. Moreover, $h$ is $C^1$, so the first factor is bounded. For the second term, observe that
$$\frac{\partial}{\partial s}\frac{\partial}{\partial x}X(x,s) = \frac{\partial f}{\partial x}(X(x,s)) \frac{\partial}{\partial x}X(x,s)$$
Let $\bar f = \max_\mO \frac{\partial f}{\partial x}$, we obtain 
$$\left|\frac{\partial }{\partial x}X(x,s) \right|\leq e^{-\bar f |s|}$$
From this, the results immediately follows with $l=\bar f$.
\flushright{\QED}
\end{proof}
Now set $\omega=(x_1, x_2)\in \mO^2$ and 
\begin{align*}
\delta_T(\omega, \lambda) & = \int_{-\infty}^0 e^{-\lambda s}\beta\big[h(X(x_1, s)) - h(X(x_2,s))\big]ds \\
 & = T_i(x_1) - T_i(x_2) \quad \forall i
\end{align*}
This function is $C^1$ in $\omega$ (as a substraction of two $C^1$ function) and holomorphic in $\lambda\in \CC_l$. Moreover, as 
$$\int_{-\infty}^0 e^{-as}\beta \big|h(X(x_1,s)) - h(X(x_2,s))\big|^2ds < +\infty$$
the Plancherel theorem can be invoked to obtain :
\begin{multline*}
    \frac{1}{2\pi}\int_{\RR}\big|\delta_T(\omega, a+i\sigma)\big|^2d\sigma \\= \int_{-\infty}^0 e^{-2as}\big|h(X(x_1,s)) - h(X(x_2,s))|^2ds
\end{multline*}

Indeed, if we define the Fourier Transform as $\hat f(\omega)=\frac{1}{\sqrt{2\pi}}\int_{\RR}f(x)e^{-i\omega x}dx$, then 
$$\delta_T(\omega, a+i\sigma) = \sqrt{2\pi} \hat f(\sigma)$$
provided that $f(s) = e^{-as}\beta\big[h(X(x_1, s)) - h(X(x_2,s))\big]\times \mathbbm{1}_{\RR^-}(s)$ where $\mathbbm{1}_{\RR^-}$ is the indicator function of $\RR^-$. 

Now note that for $\omega \in \mY$, we have $h(x_1) \neq h(x_2)$ and by continuity of the flow with respect to time, there exists a time $t_1<0$ such that $\big|h(X(x_1,s)) - h(X(x_2,s))\big|>0$.

\sj{"By continuity of the flow" ? Don't we need some hypothesis on the dynamic $\dot x = f(x)$ to affirm that ? Is the fact that $f$ is smooth enough ?}

Hence
$$\int_{\RR}\big|\delta_T(\omega, a+i\sigma)\big| > 0$$
This implies that for each $\omega\in \mY$, the function $\lambda \mapsto \delta_T(\omega, \lambda)$ is not identically zero on $\CC_l$. Then Lemma \ref{coron} gives that $\mS$ has a zero Lebesgue measure.
\flushright{\QED}
